Why and How do Complex Systems Self-Organize at All? Average Action Efficiency as a Predictor, Measure, Driver, and Mechanism of Self-Organization

Self-organization in complex systems is a process in which randomness is reduced and emergent structures appear that allow the system to function in a more competitive way with other states of the system or with other systems. It occurs only in the presence of energy gradients, facilitating energy transmission through the system and entropy production. Being a dynamic process, self-organization requires a dynamic measure and dynamic principles. The principles of decreasing unit action and increasing total action are two dynamic variational principles that are viable to utilize in a self-organizing system. Based on this, average action efficiency can serve as a quantitative measure of the degree of self-organization. Positive feedback loops connect this measure with all other characteristics of a complex system, providing all of them with a mechanism for exponential growth, and indicating power law relationships between each of them as confirmed by data and simulations. In this study, we apply those principles and the model to agent-based simulations. We find that those principles explain self-organization well and that the results confirm the model. By measuring action efficiency we can have a new answer to the question: "What is complexity and how complex is a system?". This work shows the explanatory and predictive power of those models, which can help understand and design better complex systems.

==> tex/15_powerLawFigures.tex <==


\section{Figures and Table}

This section contains the time graphs, the power law graphs, and a table with the power law fits.

\subsection{Time graphs}

In this section, we show the evolution of some of the quantities from the beginning to the end of the simulation. The phase transition from disorder initially to order can be seen. The last 200 points averaged which have been used for the power law figures can be observed. The number of ants in the runs varies from 70 to 200. The time in the simulation runs from 0 to 1000 ticks. 
\begin{figure}[H]
    \includegraphics[width=8cm]GraphsVSTime/Density_Difference.png}    \caption{The density of ants versus the time as the number of ants increases from the bottom curve to the top. As the simulation progresses, the ants become more dense.}
    \label{density}
\end{figure}

The data here show the whole run as the density increases with time as self-organization occurs. The more ants, the larger the density. The increase of density depends on two factors: 1. The shorter average path length at the end, and 2. the increased number of ants.

\begin{figure}[H]
    \includegraphics[width=8cm]GraphsVSTime/Entropy_Difference.png}    \caption{The entropy of the simulation versus the time as the number of ants increases from bottom to top. Entropy decreases from the initial random state as the path forms.}
    \label{entropy}
\end{figure}

The initial entropy when the ants are randomly dispersed scales with the number of ants, since the number of microstates corresponding to the same macrostate grows, and when they form the path, the amount of decrease of entropy is larger for the larger number of ants, even though the absolute value of entropy at the end of the simulation also scales with the number of ants, since the number of microstates when the ants form the final path also scales with the number of ants. Entropy at the initial and final state of the simulation is seen to grow with the increase of the number of agents.

\begin{figure}[H]
    \includegraphics[width=8cm]GraphsVSTime/Final_Pheromone.png}    \caption{The total amount of pheromone versus the time passed as the number of ants increases from bottom to top. As the simulation progresses, there is more pheromone for the ants to follow.}
    \label{pheromone}
\end{figure}

The pheromone is a measure of the information in the system. It scales with the number of ants. Each simulation starts with zero pheromones as the ants are dispersed randomly and do not carry any pheromones, but as they start forming the path they lay pheromones from the food and nest respectively and the more ants are in the simulation, the more pheromones they carry. Larger systems contain more information as each agent is a carrier of information.
    
\begin{figure}[H]
    \includegraphics[width=8cm]GraphsVSTime/Flow_Rate.png}    \caption{The flow rate versus the time passed as the number of ants increases from bottom to top. As the simulation progresses, the ants visit the endpoints more often.}
    \label{flowRate}
\end{figure}

The number of events, which is the number of visits to the food and nest, is inversely proportional to the average path length, and respectively average path time, scales with the number of ants as expected. Initially, the number of crossings is zero but it quickly increases and is greater for the larger systems. After the ants form the shortest path, it saturates and stays close to constant for all simulations.

\subsection{Power-Law Graphs}

The next section shows all of the power law fits between all of the quantities in the model, not shown in the main text. All of them are on a log-log scale, where a straight line is a power law curve on a linear-linear scale. The range of the data for all figures is from a population of 70 to 200 ants. These graphs match the predictions of the model and confirm the power-law relationships between all of the characteristics of a complex system derived there. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Average_Action_Efficiency/Average_Path_Time_VS_Average_Action_Efficiency.png}    \caption{The average action efficiency at the end of the simulation versus the time required to traverse the path as the number of ants increases. Action efficiency increases as the time to reach the destination shortens, i.e. the path length becomes shorter.}
    \label{a-A}
\end{figure}

In complex systems, as the agents find shorter paths, this state is more stable in dynamic equilibrium and is preserved. It has a higher probability of persisting. It is memorized by the system. If there is friction in the system, this trend will become even stronger, as the energy spent to traverse the shorter path will also decrease. To the macro-state at each point, there are many micro-states, corresponding to the variations of the paths of individual agents.

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Density_Difference_VS_Average_Action_Efficiency/Density_Difference_VS_Average_Action_Efficiency.png}    \caption{The average action efficiency at the end of the simulation versus the density increase measured as the difference between the final density minus the initial density as the number of ants increases. As the ants get more dense, they become more action efficient.}
    \label{a-p}
\end{figure}

Density increases the probability of shorter paths, i.e. less time to reach the destination, i.e. larger action efficiency. In natural systems as density increases, action efficiency increases, i.e. level of organization increases. Another term for density is concentration. When hydrogen gas clouds in the universe under the influence of gravity concentrate into stars, nucleosynthesis starts and the evolution of cosmic elements begins. In chemistry increased concentration of reactants speeds up chemical reactions, i.e. they become more action efficient. When single-cell organisms concentrate in colonies and later in multicellular organisms their level of organization increases. When human populations concentrate in cities, action efficiency increases, and civilization advances.

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Entropy_Difference_VS_Average_Action_Efficiency/Entropy_Difference_VS_Average_Action_Efficiency.png}    \caption{The average action efficiency at the end of the simulation versus the absolute amount of entropy decreases as the number of ants increases. As the ants get less random, they become more action-efficient. }
    \label{a-s}
\end{figure}

As statistical Boltzmann entropy decreases, the density (concentration) increases and this allows the system to be more action-efficient and organized. Decreased randomness is correlated with a well-formed path as a flow channel, which corresponds to the structure (organization) of the system. Here, the decrease of entropy obeys the predictions of the model being in a strict power law dependence on the other characteristics of the self-organizing complex system.

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Flow_Rate_VS_Average_Action_Efficiency/Flow_Rate_VS_Average_Action_Efficiency.png}    \caption{The average action efficiency at the end of the simulation versus the flow rate as the number of ants increases. As the ants visit the endpoints more often, they become more efficient.}
    \label{a-f}
\end{figure}
The flow rate measures the number of events in a system. For real systems, those can be nuclear or chemical reactions, computations, or anything else. In this simulation, it is the number of visits at the endpoints, or the number of crossings. As the speed of the ants is a constant in this simulation, the number of visits or the flow of events is inversely proportional to the time for crossing, i.e. the path length, therefore action efficiency increases with the number of visits.


\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Final_Pheromone_VS_Average_Action_Efficiency/Final_Pheromone_VS_Average_Action_Efficiency.png}    \caption{The average action efficiency at the end of the simulation versus the amount of pheromone, or information, as the number of ants increases. As there is more information for the ants to follow, they become more efficient.}
    \label{a-i}
\end{figure}

The pheromone is what instructs the ants how to move. They follow its gradient towards the food or the nest. As the ants form the path, they concentrate more pheromone on the trail, and they lay it faster so it has less time to evaporate. Both depend on each other in a positive feedback loop. This leads to increased action efficiency, with a power-law dependence as predicted by the model. In other complex systems, the analog of the pheromone can be temperature and catalysts in chemical reactions. In an ecosystem, as animals traverse a path, the path itself carries information, and clearing the path reduces obstacles and, therefore the time and energy to reach the destination, i.e. action.



\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Total_Action/Population_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the number of ants. As more ants are added, there is action energy within the system.}
    \label{Q-n}
\end{figure}

The total action is the sum of the actions of each agent. As the number of agents grows the total action grows.  This graph demonstrates the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Total_Action/Average_Path_Time_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the time required to traverse the path as the number of ants increases.}
    \label{Q-A}
\end{figure}

With more ants, the path forms better and gets shorter, which increases the number of visits. The shorter time is connected to more visits and increased size of the system, which is why the total action increases. This graph also demonstrates the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Density_Difference_VS_Total_Action/Density_Difference_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the increase of density as the number of ants increases. As the ants become more dense, there is more action in the system.}
    \label{Q-p}
\end{figure}

The larger the system is, it contains more agents, which corresponds to greater density, more trajectories, and more total action. This graph demonstrates as well the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Entropy_Difference_VS_Total_Action/Entropy_Difference_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the absolute decrease of entropy as the number of ants increases. As the entropy decreases, there is more action within the system.}
    \label{Q-s}
\end{figure}

As the total entropy difference increases, which means that the decrease of the internal entropy is greater for a larger number of ants, the total action increases, because there are more agents in the system and they visit the nodes more often. Greater organization of the system is correlated with more total action demonstrating again the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Flow_Rate_VS_Total_Action/Flow_Rate_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the flow rate as the number of ants increases. As the ants visit the endpoints more often, there is more total action within the system.}
    \label{Q-f}
\end{figure}

As the flow of events increases, which is the number of crossings of ants between the food and nest, the total action increases, because there are more agents in the system and they visit the nodes more often by forming a shorter path. This also demonstrates the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Final_Pheromone_VS_Total_Action/Final_Pheromone_VS_Total_Action.png}    \caption{The total action at the end of the simulation versus the amount of pheromone as the number of ants increases. As there is more information for the ants to follow, there is more action within the system.}
    \label{Q-i}
\end{figure}

As the total number of agents in the system increases, they leave more pheromones, which causes forming a shorter path, increases the number of visits, and the total action increases. Again, this graph demonstrates the principle of increasing total action in self-organization, growth, evolution, and development of systems. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Final_Pheromone/Population_VS_Final_Pheromone.png}    \caption{The total pheromone at the end of the simulation versus the number of ants. As more ants are added to the simulation, there is more information for the ants to follow.}
    \label{i-N}
\end{figure}

As the total number of ants in the system increases, they leave more pheromones and form a shorter path, which counters the evaporation of the pheromones. This increases the amount of information in the system, which helps with its rate and degree of self-organization.

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Final_Pheromone/Average_Path_Time_VS_Final_Pheromone.png}    \caption{The total pheromone at the end of the simulation versus the time required to traverse the path as the number of ants increases. As it takes less time for the ants to travel between the nodes, there is more information for the ants to follow. }
    \label{i-A}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, and as they visit the food and nest more often and there are greater number of ants they leave more pheromones. The increased amount of information in turn helps form an even shorter path which reduces the pheromone evaporation increasing the pheromones event more. This is a visualization of the result of this positive feedback loop.

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Density_Difference_VS_Final_Pheromone/Density_Difference_VS_Final_Pheromone.png}    \caption{The total pheromone at the end of the simulation versus the density increase as the number of ants increases. As the ants become more dense, there is more information for them to follow.}
    \label{i-p}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, and as there are more ants, their density increases, and as they visit the food and nest more often and there is a greater number of ants and lower evaporation, they leave more information. 


\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Entropy_Difference_VS_Final_Pheromone/Entropy_Difference_VS_Final_Pheromone.png}    \caption{The total pheromone at the end of the simulation versus the absolute decrease of entropy as the number of ants increases. As the entropy decreases, there is more information for the ants to follow.}
    \label{i-s}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher.  As there are more ants, the entropy difference increases. The entropy during each simulation decreases, and as they visit the food and nest more often and there is a greater number of ants and less evaporation they accumulate more pheromones. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Flow_Rate_VS_Final_Pheromone/Flow_Rate_VS_Final_Pheromone.png}    \caption{The total pheromone at the end of the simulation versus the flow rate as the number of ants increases. }
    \label{i-f}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher. They visit the food and nest more often, and as there are more ants, the number of visits increases proportionally, the evaporation decreases, and they accumulate more pheromones. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Flow_Rate/Population_VS_Flow_Rate.png}    \caption{The flow rate at the end of the simulation versus the number of ants. As more ants are added to the simulation and they are forming shorter paths in self-organization, the ants are visiting the endpoints more often.}
    \label{f-N}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, visit the food and nest more often, and the number of visits increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Flow_Rate/Average_Path_Time_VS_Flow_Rate.png}    \caption{The flow rate at the end of the simulation versus the time required to traverse between the nodes as the number of ants increases. As the path becomes shorter, the ants are visiting the endpoints more often.}
    \label{f-A}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, visit the food and nest more often, and as there are more ants, the number of visits increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Density_Difference_VS_Flow_Rate/Density_Difference_VS_Flow_Rate.png}    \caption{The flow rate at the end of the simulation versus the increase of density as the number of ants increases. As the ants get more dense, they are visiting the endpoints more often.}
    \label{f-p}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, this leads to an increase in density, and as there are more ants, the number of visits increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Entropy_Difference_VS_Flow_Rate/Entropy_Difference_VS_Flow_Rate.png}    \caption{The flow rate at the end of the simulation versus the absolute decrease of entropy as the number of ants increases. As the entropy decreases more, the ants are visiting the endpoints more often.}
    \label{f-s}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, the absolute decrease of entropy is larger, and as there are more ants, the number of visits increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Entropy_Difference/Population_VS_Entropy_Difference.png}    \caption{The absolute amount of entropy decrease versus the number of ants. As more ants are added to the simulation, there is a larger decrease in entropy reflecting a greater degree of self-organization.}
    \label{s-N}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, they start with a larger initial entropy and the difference between the initial and final entropy grows. More ants correspond to greater internal entropy decrease, which is one measure of self-organization. It is one of the scaling laws in the size-complexity rule. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Entropy_Difference/Average_Path_Time_VS_Entropy_Difference.png}    \caption{The absolute amount of entropy decrease versus the time required to traverse the path at the end of the simulation as the number of ants increases. As it takes more time to move between the nodes with fewer ants, there is less of a decrease in entropy.}
    \label{s-A}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher. When the path is shorter, this corresponds to shorter times to cross between the two nodes, the internal entropy decreases more. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Density_Difference_VS_Entropy_Difference/Density_Difference_VS_Entropy_Difference.png}    \caption{The absolute amount of entropy decrease versus the amount of density increase as the number of ants increases. As the ants become more dense, there is a larger decrease in entropy.}
    \label{s-p}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, and as there are more ants their density increases, and the internal entropy difference increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Density_Difference/Population_VS_Density_Difference.png}    \caption{The amount of density increase versus the number of ants. As more ants are added to the simulation, there is a larger increase in density.}
    \label{p-N}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, and as there are more ants, the density increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Average_Path_Time_VS_Density_Difference/Average_Path_Time_VS_Density_Difference.png}    \caption{The amount of density increase versus the time required to traverse the path as the number of ants increases. When there are more ants it takes less time to traverse the path, and there is more of an increase in density.}
    \label{p-A}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, visit the food and nest more often, the time to cross between the nodes decreases, and the density increases proportionally. 

\begin{figure}[H]
    \includegraphics[width=8cm]AveragedGraphs/Population_VS_Average_Path_Time/Population_VS_Average_Path_Time.png}    \caption{The time required to traverse the path versus the number of ants. As more ants are added to the simulation, it takes less time to move between the nodes.}
    \label{A-N}
\end{figure}

As the total number of ants in the system increases, they form a shorter path as the degree of self-organization is higher, visit the food and nest more often, and as there are more ants, the time for the visits decreases proportionally.

\begin{figure}[H]
    \includegraphics[width=8cm]Figures/Population_VS_Final_Entropy.png}    \caption{Population versus the average entropy at the end of the simulation. As the population increases, there is more entropy.}
    \label{FinEnt}
\end{figure}
The final entropy in the system increases when there are more agents, and therefore more possible microstates of the system. This is an expression of the unit-total duality of entropy when the total entropy in the system tends to increase with its growth. 
\begin{figure}[H]
    \includegraphics[width=8cm]Figures/Population_VS_Initial_Entropy.png}    \caption{Population versus the initial entropy on the first tick of the simulation. As the population increases, there is more entropy.}
    \label{InitEnt}
\end{figure}
The initial entropy reflects the larger number of agents in a fixed initial size of the system and scales with the size of the system as expected. The initial entropy in the system increases when there are more agents in the space of the simulation, and therefore more possible microstates of the system.
\begin{figure}[H]
    \includegraphics[width=8cm]Figures/UnitEntropyVsPopulation.png}    \caption{Unit entropy at the end of the simulation versus population. As there are more agents, there is less entropy per path at the end of the simulation.}
    \label{UnitEntVsPop}
\end{figure}
This is an expression of the unit-total duality of entropy when the unit entropy in the system tends to decrease with its growth. 


\newpage

In the next table we show the values of the fit parameters for the power law relationships

\captionsetup[table]{font={up}}

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{|l|l|l|l|} \hline
        variables&a&b&$R^{2}$\\ \hline
        $\langle\alpha\rangle$\ vs.\ Q&$7.713\cdot 10^{-36}$&$6.787\cdot 10^{-2}$&$0.977$\\ \hline
        $\langle\alpha\rangle$\ vs.\ i&$1.042\cdot 10^{-35}$&$6.131\cdot 10^{-2}$&$0.981$\\ \hline
        $\langle\alpha\rangle$\ vs.\ $\phi$&$1.510\cdot 10^{-35}$&$6.055\cdot 10^{-2}$&$0.982$\\ \hline
        $\langle\alpha\rangle$\ vs.\ $\Delta s$&$1.020\cdot 10^{-35}$&$6.675\cdot 10^{-2}$&$0.978$\\ \hline
        $\langle\alpha\rangle$\ vs.\ $\Delta\rho$&$1.647\cdot 10^{-35}$&$5.947\cdot 10^{-2}$&$0.964$\\ \hline
        $\langle\alpha\rangle$\ vs.\ $\langle t \rangle$&$1.622\cdot 10^{-34}$&$-6.175\cdot 10^{-1}$&$0.995$\\ \hline
        $\langle\alpha\rangle$\ vs.\ N&$1.168\cdot 10^{-35}$&$6.673\cdot 10^{-2}$&$0.977$\\ \hline
        Q\ vs.\ i&$8.502\cdot 10^{1}$&$9.012\cdot 10^{-1}$&$1.000$\\ \hline
        Q\ vs.\ $\phi$&$2.000\cdot 10^{4}$&$8.897\cdot 10^{-1}$&$1.000$\\ \hline
        Q\ vs.\ $\Delta s$&$6.202\cdot 10^{1}$&$9.829\cdot 10^{-1}$&$0.999$\\ \hline
        Q\ vs.\ $\Delta\rho$&$7.133\cdot 10^{4}$&$8.784\cdot 10^{-1}$&$0.990$\\ \hline
        Q\ vs.\ $\langle t \rangle$&$1.410\cdot 10^{19}$&$-8.888$&$0.972$\\ \hline
        Q\ vs.\ N&$4.550\cdot 10^{2}$&$9.830\cdot 10^{-1}$&$1.000$\\ \hline
        i\ vs.\ $\phi$&$4.281\cdot 10^{2}$&$9.873\cdot 10^{-1}$&$1.000$\\ \hline
        i\ vs.\ $\Delta s$&$7.064\cdot 10^{-1}$&$1.090$&$0.999$\\ \hline
        i\ vs.\ $\Delta\rho$&$1.755\cdot 10^{3}$&$9.740\cdot 10^{-1}$&$0.988$\\ \hline
        i\ vs.\ $\langle t \rangle$&$1.407\cdot 10^{19}$&$-9.887$&$0.976$\\ \hline
        i\ vs.\ N&$6.445$&$1.090$&$0.999$\\ \hline
        $\phi$\ vs.\ $\Delta s$&$1.521\cdot 10^{-3}$&$1.104$&$0.999$\\ \hline
        $\phi$\ vs.\ $\Delta\rho$&$4.175$&$9.864\cdot 10^{-1}$&$0.988$\\ \hline
        $\phi$\ vs.\ $\langle t \rangle$&$5.438\cdot 10^{16}$&$-1.002\cdot 10^{1}$&$0.977$\\ \hline
        $\phi$\ vs.\ N&$1.427\cdot 10^{-2}$&$1.104$&$0.999$\\ \hline
        $\Delta s$\ vs.\ $\Delta\rho$&$1.301\cdot 10^{3}$&$8.939\cdot 10^{-1}$&$0.991$\\ \hline
        $\Delta s$\ vs.\ $\langle t \rangle$&$4.439\cdot 10^{17}$&$-9.035$&$0.969$\\ \hline
        $\Delta s$\ vs.\ N&$7.598$&$1.000$&$1.000$\\ \hline
        $s_{i}$\ vs.\ N&$7.598$&$1.000$&$1.000$\\ \hline
        $s_{f}$\ vs.\ N&$5.793$&$9.745\cdot 10^{-1}$&$1.000$\\ \hline
        $s_{u}$\ vs.\ N&$4.059\cdot 10^{2}$&$-1.298\cdot 10^{-1}$&$0.938$\\ \hline
        $s_{u}$\ vs.\ $s_{f}$&$5.121\cdot 10^{2}$&$-1.329\cdot 10^{-1}$&$0.935$\\ \hline
        $\Delta\rho$\ vs.\ $\langle t \rangle$&$1.103\cdot 10^{16}$&$-9.975$&$0.949$\\ \hline
        $\Delta\rho$\ vs.\ N&$3.308\cdot 10^{-3}$&$1.110$&$0.991$\\ \hline
        $\langle t \rangle$\ vs.\ N&$7.061\cdot 10^{1}$&$-1.075\cdot 10^{-1}$&$0.970$\\ \hline
    \end{tabular}
    \vspace{5pt}
    \label{tab:fitTable}
    \caption{This table contains all the fits for the power-law graphs. The "a" and "b" values in each row follow the equation $y = ax^{b}$, and the $R^{2}$ is shown in the last column.}
\end{table}

